Hyperbolic Image-and-Pointcloud Contrastive Learning for 3D Classification

3D contrastive representation learning has exhibited remarkable efficacy across various downstream tasks. However, existing contrastive learning paradigms based on cosine similarity fail to deeply explore the potential intra-modal hierarchical and cross-modal semantic correlations about multi-modal data in Euclidean space. In response, we seek solutions in hyperbolic space and propose a hyperbolic image-and-pointcloud contrastive learning method (HyperIPC). For the intra-modal branch, we rely on the intrinsic geometric structure to explore the hyperbolic embedding representation of point cloud to capture invariant features. For the cross-modal branch, we leverage images to guide the point cloud in establishing strong semantic hierarchical correlations. Empirical experiments underscore the outstanding classification performance of HyperIPC. Notably, HyperIPC enhances object classification results by 2.8% and few-shot classification outcomes by 5.9% on ScanObjectNN compared to the baseline. Furthermore, ablation studies and confirmatory testing validate the rationality of HyperIPC's parameter settings and the effectiveness of its submodules.

==> Tables/table2.tex <==
\begin{table}[h]
\centering \small
\caption{\textbf{Comparison of ScanObjectNN linear classification results with previous self-supervised methods.} CrossPoint shows consistent improvements over prior works in both PointNet and DGCNN backbones. This illustrates the effectiveness of our approach in real-world setting.}
\label{table:scanobjectnn_cls}
\begin{tabular}{l|cc}
    \bottomrule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}}
        & \multicolumn{2}{c}{Backbone} \\
    \cline{2-3}
        & PointNet  & DGCNN\\
    \toprule \bottomrule
    Jigsaw  & 55.2 & 59.5 \\
    OcCo  & 69.5 & 78.3 \\
    STRL  & 74.2 & 77.9 \\
    CrossPoint  & 75.6 & 81.7 \\
    CrossNet  & 76.8 & 83.9 \\
    \textbf{ (Ours)} & \textbf{76.8} & \textbf{84.2}\\
    \toprule
\end{tabular}
\end{table}


==> Tables/table4.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Few-shot object classification results on ScanObjectNN.} We report mean and standard error over 10 runs. Top results of each backbone is colored in red and blue. Proposed CrossPoint improves the few-shot accuracy in all the reported settings. Table is an extended version from \cite{occo}}
\scalebox{0.93}{\label{table:scan_fsl}
\begin{tabular}{l|cccc}
\bottomrule \multicolumn{1}{c|}{\multirow{2}{*}{Method}}  & 
\multicolumn{2}{c}{5-way} & \multicolumn{2}{c}{10-way} \\\cline{2-5}
& 10-shot & 20-shot & 10-shot & 20-shot \\ \toprule \bottomrule
PointNet + Rand & 57.6$\pm$2.5 & 61.4$\pm$2.4 & 41.3$\pm$1.3 & 43.8$\pm$1.9 \\
PointNet + Jigsaw \cite{jigsaw} & 58.6$\pm$1.9 & 67.6$\pm$2.1 & 53.6$\pm$1.7 & 48.1$\pm$1.9\\
PointNet + cTree \cite{ctree}& 59.6$\pm$2.3 & 61.4$\pm$1.4 & 53.0$\pm$1.9 & 50.9$\pm$2.1 \\
PointNet + OcCo \cite{occo}& \textcolor{red}{70.4$\pm$3.3} & 72.2$\pm$3.0 & 54.8$\pm$1.3 & 61.8$\pm$1.2 \\
\textbf{PointNet + CrossPoint} & 68.2$\pm$1.8 & \textcolor{red}{73.3$\pm$2.9} & \textcolor{red}{58.7$\pm$1.8} & \textcolor{red}{64.6$\pm$1.2} \\\hline
DGCNN + Rand & 62.0$\pm$5.6 & 67.8$\pm$5.1 & 37.8$\pm$4.3 & 41.8$\pm$2.4\\
DGCNN + Jigsaw \cite{jigsaw}& 65.2$\pm$3.8 & 72.2$\pm$2.7 & 45.6$\pm$3.1 & 48.2$\pm$2.8\\
DGCNN + cTree \cite{ctree} & 68.4$\pm$3.4 & 71.6$\pm$2.9 & 42.4$\pm$2.7 & 43.0$\pm$3.0\\
DGCNN + OcCo \cite{occo} & 72.4$\pm$1.4 & 77.2$\pm$1.4 & 57.0$\pm$1.3 & 61.6$\pm$1.2\\
DGCNN + CrossPoint \cite{occo} & 74.8$\pm$1.5 & 79.0$\pm$1.2 & 62.9$\pm$1.7 & 73.9$\pm$2.2\\
\textbf{DGCNN + Ours} & \textcolor{blue}{79.6$\pm$7.6} &\textcolor{blue}{86.0$\pm$6.0} & \textcolor{blue}{68.0$\pm$4.6} & \textcolor{blue}{75.7$\pm$3.5}\\
\toprule \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_c.tex <==
\begin{table}[h]
    \centering
    \caption{\textbf{Linear classification results on ModelNet40 with varying number of rendered 2D images (n).} CrossPoint with single corresponding image performs better than or equal to multiple rendered images. We choose n=1 for all the experiments.}
    \label{tab:multiple_images}
    \begin{tabular}{cccccc}
    \toprule
    \begin{tabular}{l}No. of rendered\\2D images (n)\end{tabular} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5}\\ \hline
    Linear Accuracy & \textbf{91.2} & 91.2 & 90.9 & 91.0 & 90.5 \\ 
    \bottomrule
    \end{tabular}
\end{table}
